Neural-Network-based Viscosity Closure for Non-Newtonian Multiphase Flows

Materials used in polymer-based additive manufacturing processes, such as Digital Light Processing (DLP) and direct ink writing (DIW), typically exhibit non-Newtonian rheology. Carreau-Yasuda and power-law models describe basic shear-thinning and shear-thickening behavior well, but applying them to a new material requires choosing a functional form, deriving it, and re-implementing it inside the flow solver. We present a deployment workflow in which a neural network trained on experimental rheometry data serves as the viscosity closure inside a Cahn-Hilliard-Navier-Stokes (CHNS) finite element solver. The learned closure is generalized Newtonian: viscosity depends only on the local shear rate at the current instant. Lipschitz regularization during training produces smooth viscosity predictions, and the trained network is exported in the Open Neural Network Exchange (ONNX) format and queried by the solver at runtime via the ONNX runtime, without solver modification or network reimplementation. The framework is built on a parallel octree-based adaptive mesh refinement infrastructure that concentrates resolution at the fluid interface. We validate the CHNS solver against benchmark shear-thinning bubble-rise cases from the literature, reproducing reported bubble shapes across varying power-law indices and Weber numbers. We characterized two silicone ink formulations, recorded their rise dynamics in perfluorodecalin on high-speed video, and used the resulting data to test the full workflow. Simulated rise velocities fall within the experimentally measured spread, and the simulated steady-state droplet shape agrees with the observed one. This work contributes to a growing body of literature on integrating neural constitutive closures into multiphysics simulations, and demonstrates a practical path for deploying experimentally trained rheological surrogates inside finite element solvers.

==> SyntheticAN_Phi_150.tex <==
phi,x,y,z
0,1.9375,1.7496,0
0,1.9343,1.75,0
0,1.9414,1.7491,0
0,1.9453,1.7486,0
0,1.9492,1.7482,0
0,1.9531,1.7478,0
0,1.957,1.7474,0
0,1.9609,1.7471,0
0,1.9648,1.7468,0
0,1.9688,1.7465,0
0,1.9766,1.7461,0
0,1.9762,1.7461,0
0,1.9727,1.7463,0
0,1.9805,1.7459,0
0,1.9844,1.7458,0
0,1.9883,1.7456,0
0,1.9922,1.7456,0
0,1.9961,1.7455,0
0,2,1.7455,0
0,1.6875,1.8592,0
0,1.6873,1.8594,0
0,1.6719,1.8727,0
0,1.6694,1.875,0
0,1.6797,1.8658,0
0,1.6781,1.8672,0
0,1.6836,1.8625,0
0,1.6826,1.8633,0
0,1.6758,1.8692,0
0,1.6737,1.8711,0
0,1.7188,1.8352,0
0,1.7177,1.8359,0
0,1.707,1.8437,0
0,1.707,1.8438,0
0,1.7109,1.8409,0
0,1.7148,1.838,0
0,1.7123,1.8398,0
0,1.7305,1.8272,0
0,1.7291,1.8281,0
0,1.7344,1.8246,0
0,1.7422,1.8197,0
0,1.7411,1.8203,0
0,1.75,1.8149,0
0,1.7475,1.8164,0
0,1.7461,1.8173,0
0,1.7383,1.8221,0
0,1.735,1.8242,0
0,1.7266,1.8298,0
0,1.7233,1.832,0
0,1.7227,1.8325,0
0,1.7031,1.8467,0
0,1.7019,1.8477,0
0,1.6992,1.8497,0
0,1.6969,1.8516,0
0,1.6953,1.8528,0
0,1.692,1.8555,0
0,1.6914,1.856,0
0,1.625,1.9213,0
0,1.6245,1.9219,0
0,1.6213,1.9258,0
0,1.6211,1.926,0
0,1.6181,1.9297,0
0,1.6172,1.9308,0
0,1.615,1.9336,0
0,1.6133,1.9358,0
0,1.6119,1.9375,0
0,1.5938,1.9626,0
0,1.5923,1.9648,0
0,1.5898,1.9685,0
0,1.5897,1.9688,0
0,1.6094,1.9408,0
0,1.6089,1.9414,0
0,1.606,1.9453,0
0,1.6016,1.9514,0
0,1.6003,1.9531,0
0,1.6055,1.9461,0
0,1.6032,1.9492,0
0,1.5977,1.957,0
0,1.5976,1.957,0
0,1.5949,1.9609,0
0,1.5859,1.9745,0
0,1.5847,1.9766,0
0,1.5871,1.9727,0
0,1.5822,1.9805,0
0,1.582,1.9808,0
0,1.5798,1.9844,0
0,1.5781,1.9872,0
0,1.5775,1.9883,0
0,1.5752,1.9922,0
0,1.5742,1.9939,0
0,1.573,1.9961,0
0,1.5708,2,0
0,1.6562,1.8875,0
0,1.6531,1.8906,0
0,1.6406,1.9036,0
0,1.6382,1.9062,0
0,1.6484,1.8954,0
0,1.6455,1.8984,0
0,1.6523,1.8914,0
0,1.6493,1.8945,0
0,1.6445,1.8994,0
0,1.6418,1.9023,0
0,1.6641,1.88,0
0,1.6611,1.8828,0
0,1.668,1.8763,0
0,1.6652,1.8789,0
0,1.6602,1.8837,0
0,1.657,1.8867,0
0,1.6328,1.9122,0
0,1.6312,1.9141,0
0,1.6367,1.9079,0
0,1.6347,1.9102,0
0,1.6289,1.9167,0
0,1.6278,1.918,0
0,1.7578,1.8103,0
0,1.754,1.8125,0
0,1.7617,1.8081,0
0,1.7608,1.8086,0
0,1.7656,1.8059,0
0,1.7695,1.8038,0
0,1.7679,1.8047,0
0,1.7734,1.8017,0
0,1.7773,1.7997,0
0,1.7752,1.8008,0
0,1.7812,1.7977,0
0,1.7852,1.7957,0
0,1.7829,1.7969,0
0,1.7891,1.7939,0
0,1.793,1.792,0
0,1.7909,1.793,0
0,1.7969,1.7902,0
0,1.8008,1.7884,0
0,1.7993,1.7891,0
0,1.8047,1.7867,0
0,1.8086,1.785,0
0,1.8081,1.7852,0
0,1.8125,1.7833,0
0,1.8203,1.7801,0
0,1.8175,1.7812,0
0,1.8281,1.7771,0
0,1.8274,1.7773,0
0,1.8242,1.7786,0
0,1.8398,1.7728,0
0,1.838,1.7734,0
0,1.8438,1.7715,0
0,1.832,1.7756,0
0,1.8359,1.7742,0
0,1.8633,1.7652,0
0,1.862,1.7656,0
0,1.8672,1.7641,0
0,1.8711,1.763,0
0,1.875,1.762,0
0,1.8516,1.7689,0
0,1.8495,1.7695,0
0,1.8477,1.7701,0
0,1.8555,1.7676,0
0,1.8594,1.7664,0
0,1.8164,1.7817,0
0,1.7539,1.8126,0
0,1.8789,1.7609,0
0,1.8759,1.7617,0
0,1.8828,1.7599,0
0,1.8867,1.759,0
0,1.8906,1.7581,0
0,1.8945,1.7572,0
0,1.8917,1.7578,0
0,1.8984,1.7563,0
0,1.9023,1.7555,0
0,1.9062,1.7547,0
0,1.9141,1.7532,0
0,1.9104,1.7539,0
0,1.9102,1.7539,0
0,1.918,1.7525,0
0,1.9219,1.7519,0
0,1.9258,1.7513,0
0,1.9297,1.7507,0
0,1.9336,1.7501,0
0,2.0039,1.7455,0
0,2.0078,1.7456,0
0,2.0117,1.7456,0
0,2.0156,1.7458,0
0,2.0195,1.7459,0
0,2.0234,1.7461,0
0,2.0238,1.7461,0
0,2.0273,1.7463,0
0,2.0312,1.7465,0
0,2.0352,1.7468,0
0,2.0391,1.7471,0
0,2.043,1.7474,0
0,2.0469,1.7478,0
0,2.0508,1.7482,0
0,2.0547,1.7486,0
0,2.0586,1.7491,0
0,2.0625,1.7496,0
0,2.0657,1.75,0
0,2.0664,1.7501,0
0,2.0703,1.7507,0
0,2.0742,1.7513,0
0,2.0781,1.7519,0
0,2.082,1.7525,0
0,2.0859,1.7532,0
0,2.0897,1.7539,0
0,2.0898,1.7539,0
0,2.0938,1.7547,0
0,2.0977,1.7555,0
0,2.1016,1.7563,0
0,2.1055,1.7572,0
0,2.1083,1.7578,0
0,2.1094,1.7581,0
0,2.1133,1.759,0
0,2.1172,1.7599,0
0,2.1211,1.7609,0
0,2.1241,1.7617,0
0,2.125,1.762,0
0,2.1289,1.763,0
0,2.1328,1.7641,0
0,2.1367,1.7652,0
0,2.138,1.7656,0
0,2.1406,1.7664,0
0,2.1445,1.7676,0
0,2.1484,1.7689,0
0,2.1505,1.7695,0
0,2.1523,1.7701,0
0,2.1562,1.7714,0
0,2.1602,1.7728,0
0,2.162,1.7734,0
0,2.1641,1.7742,0
0,2.168,1.7756,0
0,2.1719,1.7771,0
0,2.1726,1.7773,0
0,2.1758,1.7786,0
0,2.1797,1.7801,0
0,2.1825,1.7812,0
0,2.1836,1.7817,0
0,2.1875,1.7833,0
0,2.1914,1.7849,0
0,2.1919,1.7852,0
0,2.1953,1.7867,0
0,2.1992,1.7884,0
0,2.2007,1.7891,0
0,2.2031,1.7902,0
0,2.207,1.792,0
0,2.2091,1.793,0
0,2.2109,1.7938,0
0,2.2148,1.7957,0
0,2.2171,1.7969,0
0,2.2188,1.7977,0
0,2.2227,1.7997,0
0,2.2248,1.8008,0
0,2.2266,1.8017,0
0,2.2305,1.8038,0
0,2.2321,1.8047,0
0,2.2344,1.8059,0
0,2.2383,1.8081,0
0,2.2392,1.8086,0
0,2.2422,1.8103,0
0,2.246,1.8125,0
0,2.2461,1.8126,0
0,2.25,1.8149,0
0,2.2525,1.8164,0
0,2.2539,1.8172,0
0,2.2578,1.8196,0
0,2.2589,1.8203,0
0,2.2617,1.8221,0
0,2.265,1.8242,0
0,2.2656,1.8246,0
0,2.2695,1.8272,0
0,2.2709,1.8281,0
0,2.2734,1.8298,0
0,2.2767,1.832,0
0,2.2773,1.8325,0
0,2.2812,1.8352,0
0,2.2823,1.8359,0
0,2.2852,1.838,0
0,2.2877,1.8398,0
0,2.2891,1.8408,0
0,2.293,1.8437,0
0,2.293,1.8438,0
0,2.2969,1.8467,0
0,2.2982,1.8477,0
0,2.3008,1.8497,0
0,2.3031,1.8516,0
0,2.3047,1.8528,0
0,2.308,1.8555,0
0,2.3086,1.8559,0
0,2.3125,1.8591,0
0,2.3128,1.8594,0
0,2.3164,1.8624,0
0,2.3174,1.8633,0
0,2.3203,1.8658,0
0,2.3219,1.8672,0
0,2.3242,1.8692,0
0,2.3263,1.8711,0
0,2.3281,1.8727,0
0,2.3307,1.875,0
0,2.332,1.8763,0
0,2.3349,1.8789,0
0,2.3359,1.8799,0
0,2.339,1.8828,0
0,2.3398,1.8836,0
0,2.343,1.8867,0
0,2.3438,1.8875,0
0,2.3469,1.8906,0
0,2.3477,1.8914,0
0,2.3508,1.8945,0
0,2.3516,1.8953,0
0,2.3545,1.8984,0
0,2.3555,1.8994,0
0,2.3582,1.9023,0
0,2.3594,1.9036,0
0,2.3618,1.9062,0
0,2.3633,1.9078,0
0,2.3654,1.9102,0
0,2.3672,1.9122,0
0,2.3688,1.9141,0
0,2.3711,1.9167,0
0,2.3722,1.918,0
0,2.375,1.9213,0
0,2.3755,1.9219,0
0,2.3787,1.9258,0
0,2.3789,1.926,0
0,2.3819,1.9297,0
0,2.3828,1.9308,0
0,2.385,1.9336,0
0,2.3867,1.9357,0
0,2.3881,1.9375,0
0,2.3906,1.9408,0
0,2.3911,1.9414,0
0,2.394,1.9453,0
0,2.3945,1.946,0
0,2.3969,1.9492,0
0,2.3984,1.9514,0
0,2.3997,1.9531,0
0,2.4023,1.9569,0
0,2.4024,1.957,0
0,2.4051,1.9609,0
0,2.4062,1.9626,0
0,2.4078,1.9648,0
0,2.4102,1.9685,0
0,2.4103,1.9688,0
0,2.4129,1.9727,0
0,2.4141,1.9745,0
0,2.4154,1.9766,0
0,2.4178,1.9805,0
0,2.418,1.9808,0
0,2.4202,1.9844,0
0,2.4219,1.9872,0
0,2.4225,1.9883,0
0,2.4248,1.9922,0
0,2.4258,1.9939,0
0,2.427,1.9961,0
0,2.4292,2,0
0,1.5625,2.0155,0
0,1.5625,2.0156,0
0,1.5605,2.0195,0
0,1.5586,2.0234,0
0,1.5586,2.0234,0
0,1.5567,2.0273,0
0,1.5548,2.0312,0
0,1.5547,2.0315,0
0,1.553,2.0352,0
0,1.5513,2.0391,0
0,1.5508,2.0401,0
0,1.5495,2.043,0
0,1.5479,2.0469,0
0,1.5469,2.0492,0
0,1.5462,2.0508,0
0,1.5446,2.0547,0
0,1.543,2.0586,0
0,1.543,2.0587,0
0,1.5415,2.0625,0
0,1.5703,2.0009,0
0,1.5686,2.0039,0
0,1.5665,2.0078,0
0,1.5664,2.0081,0
0,1.5645,2.0117,0
0,1.5312,2.0916,0
0,1.5305,2.0938,0
0,1.5391,2.0689,0
0,1.5385,2.0703,0
0,1.54,2.0664,0
0,1.5371,2.0742,0
0,1.5357,2.0781,0
0,1.5352,2.0798,0
0,1.5344,2.082,0
0,1.5331,2.0859,0
0,1.5318,2.0898,0
0,1.5293,2.0977,0
0,1.5282,2.1016,0
0,1.5273,2.1044,0
0,1.527,2.1055,0
0,1.5259,2.1094,0
0,1.5249,2.1133,0
0,1.5238,2.1172,0
0,1.5234,2.1187,0
0,1.5228,2.1211,0
0,1.5219,2.125,0
0,1.5209,2.1289,0
0,1.52,2.1328,0
0,1.5195,2.135,0
0,1.5191,2.1367,0
0,1.5183,2.1406,0
0,1.5156,2.1544,0
0,1.5153,2.1562,0
0,1.5175,2.1445,0
0,1.5167,2.1484,0
0,1.516,2.1523,0
0,1.5146,2.1602,0
0,1.514,2.1641,0
0,1.5134,2.168,0
0,1.5128,2.1719,0
0,1.5122,2.1758,0
0,1.5117,2.1797,0
0,1.5117,2.1797,0
0,1.5112,2.1836,0
0,1.5108,2.1875,0
0,1.5103,2.1914,0
0,1.51,2.1953,0
0,1.5096,2.1992,0
0,1.5093,2.2031,0
0,1.509,2.207,0
0,1.5087,2.2109,0
0,1.5085,2.2148,0
0,1.5083,2.2188,0
0,1.5081,2.2227,0
0,1.5079,2.2266,0
0,1.5078,2.2314,0
0,1.5077,2.2344,0
0,1.5078,2.2305,0
0,1.5077,2.2383,0
0,1.5077,2.2422,0
0,1.5077,2.2461,0
0,1.5077,2.25,0
0,1.5078,2.2539,0
0,1.5078,2.2548,0
0,1.5079,2.2578,0
0,1.508,2.2617,0
0,1.5082,2.2656,0
0,1.5084,2.2695,0
0,1.5086,2.2734,0
0,1.5089,2.2773,0
0,1.5091,2.2812,0
0,1.5094,2.2852,0
0,1.5098,2.2891,0
0,1.5102,2.293,0
0,1.5106,2.2969,0
0,1.511,2.3008,0
0,1.5115,2.3047,0
0,1.5117,2.3066,0
0,1.512,2.3086,0
0,1.5125,2.3125,0
0,1.5131,2.3164,0
0,1.5137,2.3203,0
0,1.5143,2.3242,0
0,1.5149,2.3281,0
0,1.5156,2.3319,0
0,1.5156,2.332,0
0,1.5164,2.3359,0
0,1.5171,2.3398,0
0,1.5179,2.3438,0
0,1.5187,2.3477,0
0,1.5195,2.3514,0
0,1.5196,2.3516,0
0,1.5205,2.3555,0
0,1.5214,2.3594,0
0,1.5223,2.3633,0
0,1.5233,2.3672,0
0,1.5234,2.3677,0
0,1.5243,2.3711,0
0,1.5254,2.375,0
0,1.5264,2.3789,0
0,1.5273,2.382,0
0,1.5276,2.3828,0
0,1.5287,2.3867,0
0,1.5299,2.3906,0
0,1.5311,2.3945,0
0,1.5312,2.3949,0
0,1.5324,2.3984,0
0,1.5337,2.4023,0
0,1.535,2.4062,0
0,1.5352,2.4066,0
0,1.5364,2.4102,0
0,1.5378,2.4141,0
0,1.5391,2.4175,0
0,1.5392,2.418,0
0,1.5407,2.4219,0
0,1.5422,2.4258,0
0,1.543,2.4276,0
0,1.5438,2.4297,0
0,1.5454,2.4336,0
0,1.5469,2.4372,0
0,1.547,2.4375,0
0,1.5487,2.4414,0
0,1.5504,2.4453,0
0,1.5508,2.4462,0
0,1.5521,2.4492,0
0,1.5539,2.4531,0
0,1.5547,2.4548,0
0,1.5557,2.457,0
0,1.5576,2.4609,0
0,1.5586,2.463,0
0,1.5595,2.4648,0
0,1.5615,2.4688,0
0,1.5625,2.4708,0
0,1.5635,2.4727,0
0,1.5655,2.4766,0
0,1.5664,2.4783,0
0,1.5676,2.4805,0
0,1.5697,2.4844,0
0,1.5703,2.4855,0
0,1.5719,2.4883,0
0,1.5741,2.4922,0
0,1.5742,2.4924,0
0,1.5764,2.4961,0
0,1.5781,2.4991,0
0,1.5787,2.5,0
0,1.581,2.5039,0
0,1.582,2.5055,0
0,1.5835,2.5078,0
0,1.5859,2.5117,0
0,1.5859,2.5118,0
0,1.5884,2.5156,0
0,1.5898,2.5178,0
0,1.591,2.5195,0
0,1.5936,2.5234,0
0,1.5938,2.5237,0
0,1.5963,2.5273,0
0,1.5977,2.5294,0
0,1.599,2.5312,0
0,1.6016,2.5349,0
0,1.6018,2.5352,0
0,1.6046,2.5391,0
0,1.6055,2.5403,0
0,1.6075,2.543,0
0,1.6094,2.5455,0
0,1.6104,2.5469,0
0,1.6133,2.5506,0
0,1.6135,2.5508,0
0,1.6165,2.5547,0
0,1.6172,2.5555,0
0,1.6197,2.5586,0
0,1.6211,2.5604,0
0,1.6229,2.5625,0
0,1.625,2.5651,0
0,1.6261,2.5664,0
0,1.6289,2.5697,0
0,1.6295,2.5703,0
0,1.6328,2.5742,0
0,1.6329,2.5742,0
0,1.6363,2.5781,0
0,1.6367,2.5785,0
0,1.6399,2.582,0
0,1.6406,2.5828,0
0,1.6435,2.5859,0
0,1.6445,2.587,0
0,1.6472,2.5898,0
0,1.6484,2.5911,0
0,1.651,2.5938,0
0,1.6523,2.5951,0
0,1.6549,2.5977,0
0,1.6562,2.599,0
0,1.6588,2.6016,0
0,1.6602,2.6029,0
0,1.6629,2.6055,0
0,1.6641,2.6066,0
0,1.667,2.6094,0
0,1.668,2.6103,0
0,1.6712,2.6133,0
0,1.6719,2.6139,0
0,1.6756,2.6172,0
0,1.6758,2.6174,0
0,1.6797,2.6208,0
0,1.68,2.6211,0
0,1.6836,2.6242,0
0,1.6845,2.625,0
0,1.6875,2.6275,0
0,1.6892,2.6289,0
0,1.6914,2.6308,0
0,1.6939,2.6328,0
0,1.6953,2.6339,0
0,1.6988,2.6367,0
0,1.6992,2.637,0
0,1.7031,2.6401,0
0,1.7038,2.6406,0
0,1.707,2.6431,0
0,1.709,2.6445,0
0,1.7109,2.646,0
0,1.7143,2.6484,0
0,1.7148,2.6488,0
0,1.7188,2.6516,0
0,1.7197,2.6523,0
0,1.7227,2.6544,0
0,1.7253,2.6562,0
0,1.7266,2.6571,0
0,1.7305,2.6597,0
0,1.7311,2.6602,0
0,1.7344,2.6623,0
0,1.7371,2.6641,0
0,1.7383,2.6648,0
0,1.7422,2.6673,0
0,1.7432,2.668,0
0,1.7461,2.6697,0
0,1.7496,2.6719,0
0,1.75,2.6721,0
0,1.7539,2.6744,0
0,1.7562,2.6758,0
0,1.7578,2.6767,0
0,1.7617,2.6789,0
0,1.763,2.6797,0
0,1.7656,2.6811,0
0,1.7695,2.6833,0
0,1.7702,2.6836,0
0,1.7734,2.6854,0
0,1.7773,2.6874,0
0,1.7775,2.6875,0
0,1.7812,2.6894,0
0,1.7852,2.6914,0
0,1.7853,2.6914,0
0,1.7891,2.6933,0
0,1.793,2.6951,0
0,1.7933,2.6953,0
0,1.7969,2.697,0
0,1.8008,2.6987,0
0,1.8018,2.6992,0
0,1.8047,2.7005,0
0,1.8086,2.7022,0
0,1.8108,2.7031,0
0,1.8125,2.7039,0
0,1.8164,2.7055,0
0,1.8202,2.707,0
0,1.8203,2.7071,0
0,1.8242,2.7086,0
0,1.8281,2.7101,0
0,1.8303,2.7109,0
0,1.832,2.7116,0
0,1.8359,2.713,0
0,1.8398,2.7144,0
0,1.8411,2.7148,0
0,1.8438,2.7158,0
0,1.8477,2.7171,0
0,1.8516,2.7183,0
0,1.8528,2.7188,0
0,1.8555,2.7196,0
0,1.8594,2.7208,0
0,1.8633,2.722,0
0,1.8656,2.7227,0
0,1.8672,2.7231,0
0,1.8711,2.7242,0
0,1.875,2.7253,0
0,1.8789,2.7263,0
0,1.8799,2.7266,0
0,1.8828,2.7273,0
0,1.8867,2.7283,0
0,1.8906,2.7292,0
0,1.8945,2.7301,0
0,1.8963,2.7305,0
0,1.8984,2.7309,0
0,1.9023,2.7318,0
0,1.9062,2.7326,0
0,1.9102,2.7333,0
0,1.9141,2.734,0
0,1.916,2.7344,0
0,1.918,2.7347,0
0,1.9219,2.7354,0
0,1.9258,2.736,0
0,1.9297,2.7366,0
0,1.9336,2.7372,0
0,1.9375,2.7377,0
0,1.9414,2.7382,0
0,1.9422,2.7383,0
0,1.9453,2.7387,0
0,1.9492,2.7391,0
0,1.9531,2.7395,0
0,1.957,2.7398,0
0,1.9609,2.7402,0
0,1.9648,2.7405,0
0,1.9688,2.7407,0
0,1.9727,2.741,0
0,1.9766,2.7412,0
0,1.9805,2.7414,0
0,1.9844,2.7415,0
0,1.9883,2.7416,0
0,1.9922,2.7417,0
0,1.9961,2.7417,0
0,2,2.7418,0
0,2.4297,2.0008,0
0,2.4314,2.0039,0
0,2.4335,2.0078,0
0,2.4336,2.008,0
0,2.4355,2.0117,0
0,2.4375,2.0155,0
0,2.4375,2.0156,0
0,2.4395,2.0195,0
0,2.4414,2.0234,0
0,2.4414,2.0234,0
0,2.4433,2.0273,0
0,2.4452,2.0312,0
0,2.4453,2.0315,0
0,2.447,2.0352,0
0,2.4487,2.0391,0
0,2.4492,2.0401,0
0,2.4505,2.043,0
0,2.4521,2.0469,0
0,2.4531,2.0492,0
0,2.4538,2.0508,0
0,2.4554,2.0547,0
0,2.457,2.0586,0
0,2.457,2.0587,0
0,2.4585,2.0625,0
0,2.46,2.0664,0
0,2.4609,2.0689,0
0,2.4615,2.0703,0
0,2.4629,2.0742,0
0,2.4643,2.0781,0
0,2.4648,2.0798,0
0,2.4656,2.082,0
0,2.4669,2.0859,0
0,2.4682,2.0898,0
0,2.4688,2.0916,0
0,2.4695,2.0938,0
0,2.4707,2.0977,0
0,2.4718,2.1016,0
0,2.4727,2.1044,0
0,2.473,2.1055,0
0,2.4741,2.1094,0
0,2.4751,2.1133,0
0,2.4762,2.1172,0
0,2.4766,2.1187,0
0,2.4772,2.1211,0
0,2.4782,2.125,0
0,2.4791,2.1289,0
0,2.48,2.1328,0
0,2.4805,2.135,0
0,2.4809,2.1367,0
0,2.4817,2.1406,0
0,2.4825,2.1445,0
0,2.4833,2.1484,0
0,2.484,2.1523,0
0,2.4844,2.1544,0
0,2.4847,2.1562,0
0,2.4854,2.1602,0
0,2.486,2.1641,0
0,2.4866,2.168,0
0,2.4872,2.1719,0
0,2.4878,2.1758,0
0,2.4883,2.1796,0
0,2.4883,2.1797,0
0,2.4888,2.1836,0
0,2.4892,2.1875,0
0,2.4897,2.1914,0
0,2.4901,2.1953,0
0,2.4904,2.1992,0
0,2.4907,2.2031,0
0,2.491,2.207,0
0,2.4913,2.2109,0
0,2.4915,2.2148,0
0,2.4918,2.2188,0
0,2.4919,2.2227,0
0,2.4921,2.2266,0
0,2.4922,2.2303,0
0,2.4922,2.2305,0
0,2.4923,2.2344,0
0,2.4923,2.2383,0
0,2.4924,2.2422,0
0,2.4923,2.2461,0
0,2.4923,2.25,0
0,2.4921,2.2578,0
0,2.4922,2.2559,0
0,2.4922,2.2539,0
0,2.492,2.2617,0
0,2.4918,2.2656,0
0,2.4916,2.2695,0
0,2.4914,2.2734,0
0,2.4912,2.2773,0
0,2.4909,2.2812,0
0,2.4906,2.2852,0
0,2.4902,2.2891,0
0,2.4899,2.293,0
0,2.4895,2.2969,0
0,2.489,2.3008,0
0,2.4886,2.3047,0
0,2.488,2.3086,0
0,2.4883,2.3068,0
0,2.4875,2.3125,0
0,2.4869,2.3164,0
0,2.4864,2.3203,0
0,2.4857,2.3242,0
0,2.4851,2.3281,0
0,2.4837,2.3359,0
0,2.4844,2.3321,0
0,2.4829,2.3398,0
0,2.4821,2.3438,0
0,2.4844,2.332,0
0,2.4813,2.3477,0
0,2.4805,2.3516,0
0,2.4805,2.3515,0
0,2.4796,2.3555,0
0,2.4786,2.3594,0
0,2.4777,2.3633,0
0,2.4767,2.3672,0
0,2.4757,2.3711,0
0,2.4766,2.3678,0
0,2.4746,2.375,0
0,2.4676,2.3984,0
0,2.4688,2.3949,0
0,2.4663,2.4023,0
0,2.465,2.4062,0
0,2.4736,2.3789,0
0,2.4724,2.3828,0
0,2.4727,2.3821,0
0,2.4713,2.3867,0
0,2.4701,2.3906,0
0,2.4689,2.3945,0
0,2.4636,2.4102,0
0,2.4648,2.4067,0
0,2.4622,2.4141,0
0,2.4608,2.418,0
0,2.4609,2.4176,0
0,2.4593,2.4219,0
0,2.453,2.4375,0
0,2.4531,2.4373,0
0,2.4578,2.4258,0
0,2.4562,2.4297,0
0,2.457,2.4277,0
0,2.4547,2.4336,0
0,2.4366,2.4727,0
0,2.4375,2.4708,0
0,2.4345,2.4766,0
0,2.4324,2.4805,0
0,2.4336,2.4783,0
0,2.4303,2.4844,0
0,2.4214,2.5,0
0,2.4219,2.4991,0
0,2.4282,2.4883,0
0,2.4297,2.4855,0
0,2.4259,2.4922,0
0,2.4237,2.4961,0
0,2.4258,2.4925,0
0,2.4514,2.4414,0
0,2.4497,2.4453,0
0,2.4479,2.4492,0
0,2.4492,2.4463,0
0,2.4461,2.4531,0
0,2.4443,2.457,0
0,2.4453,2.4549,0
0,2.4424,2.4609,0
0,2.4405,2.4648,0
0,2.4414,2.463,0
0,2.4386,2.4688,0
0,2.0039,2.7417,0
0,2.0078,2.7417,0
0,2.0117,2.7416,0
0,2.0156,2.7415,0
0,2.0195,2.7414,0
0,2.0234,2.7412,0
0,2.0273,2.741,0
0,2.0312,2.7407,0
0,2.0352,2.7405,0
0,2.0391,2.7402,0
0,2.043,2.7398,0
0,2.0469,2.7395,0
0,2.0508,2.7391,0
0,2.0547,2.7387,0
0,2.0578,2.7383,0
0,2.0586,2.7382,0
0,2.0625,2.7377,0
0,2.084,2.7344,0
0,2.0859,2.734,0
0,2.0898,2.7333,0
0,2.0938,2.7326,0
0,2.0664,2.7372,0
0,2.0703,2.7366,0
0,2.0742,2.736,0
0,2.0781,2.7354,0
0,2.082,2.7347,0
0,2.0977,2.7318,0
0,2.1016,2.731,0
0,2.1037,2.7305,0
0,2.1055,2.7301,0
0,2.1094,2.7292,0
0,2.1201,2.7266,0
0,2.1211,2.7263,0
0,2.125,2.7253,0
0,2.1133,2.7283,0
0,2.1172,2.7273,0
0,2.2225,2.6875,0
0,2.2227,2.6874,0
0,2.2266,2.6854,0
0,2.2299,2.6836,0
0,2.2305,2.6833,0
0,2.2344,2.6811,0
0,2.237,2.6797,0
0,2.2383,2.6789,0
0,2.2422,2.6767,0
0,2.2438,2.6758,0
0,2.2461,2.6744,0
0,2.25,2.6721,0
0,2.1472,2.7188,0
0,2.1484,2.7184,0
0,2.1523,2.7171,0
0,2.1562,2.7158,0
0,2.1697,2.7109,0
0,2.1719,2.7101,0
0,2.1589,2.7148,0
0,2.1602,2.7144,0
0,2.1641,2.713,0
0,2.168,2.7116,0
0,2.1758,2.7086,0
0,2.1797,2.7071,0
0,2.1798,2.707,0
0,2.1836,2.7055,0
0,2.1875,2.7039,0
0,2.1289,2.7242,0
0,2.1328,2.7231,0
0,2.1344,2.7227,0
0,2.1367,2.722,0
0,2.1406,2.7208,0
0,2.1445,2.7196,0
0,2.1892,2.7031,0
0,2.1914,2.7022,0
0,2.1953,2.7005,0
0,2.1982,2.6992,0
0,2.1992,2.6987,0
0,2.2031,2.697,0
0,2.2067,2.6953,0
0,2.207,2.6951,0
0,2.2109,2.6933,0
0,2.2147,2.6914,0
0,2.2148,2.6914,0
0,2.2188,2.6894,0
0,2.3739,2.5664,0
0,2.375,2.5651,0
0,2.3706,2.5703,0
0,2.3711,2.5697,0
0,2.3672,2.5742,0
0,2.3672,2.5742,0
0,2.3637,2.5781,0
0,2.3565,2.5859,0
0,2.3594,2.5829,0
0,2.349,2.5938,0
0,2.3516,2.5911,0
0,2.3528,2.5898,0
0,2.3555,2.5871,0
0,2.3602,2.582,0
0,2.3633,2.5786,0
0,2.3412,2.6016,0
0,2.3438,2.5991,0
0,2.333,2.6094,0
0,2.3359,2.6066,0
0,2.3372,2.6055,0
0,2.3398,2.6029,0
0,2.3245,2.6172,0
0,2.3281,2.6139,0
0,2.32,2.6211,0
0,2.3203,2.6209,0
0,2.3155,2.625,0
0,2.3164,2.6242,0
0,2.3242,2.6174,0
0,2.3288,2.6133,0
0,2.332,2.6103,0
0,2.3452,2.5977,0
0,2.3477,2.5951,0
0,2.4038,2.5273,0
0,2.4062,2.5237,0
0,2.4011,2.5312,0
0,2.4023,2.5294,0
0,2.419,2.5039,0
0,2.4166,2.5078,0
0,2.418,2.5056,0
0,2.4116,2.5156,0
0,2.4141,2.5118,0
0,2.4141,2.5117,0
0,2.4091,2.5195,0
0,2.4102,2.5179,0
0,2.4065,2.5234,0
0,2.3896,2.5469,0
0,2.3906,2.5455,0
0,2.3983,2.5352,0
0,2.3984,2.535,0
0,2.3955,2.5391,0
0,2.3926,2.543,0
0,2.3945,2.5403,0
0,2.3866,2.5508,0
0,2.3867,2.5506,0
0,2.3835,2.5547,0
0,2.3804,2.5586,0
0,2.3828,2.5556,0
0,2.3772,2.5625,0
0,2.3789,2.5604,0
0,2.2803,2.6523,0
0,2.2812,2.6516,0
0,2.2747,2.6562,0
0,2.2773,2.6544,0
0,2.2962,2.6406,0
0,2.2969,2.6401,0
0,2.3109,2.6289,0
0,2.3125,2.6275,0
0,2.3061,2.6328,0
0,2.3086,2.6308,0
0,2.3012,2.6367,0
0,2.3047,2.6339,0
0,2.3008,2.6371,0
0,2.2857,2.6484,0
0,2.2891,2.646,0
0,2.291,2.6445,0
0,2.293,2.6431,0
0,2.2852,2.6489,0
0,2.2629,2.6641,0
0,2.2656,2.6623,0
0,2.2568,2.668,0
0,2.2578,2.6673,0
0,2.2504,2.6719,0
0,2.2539,2.6697,0
0,2.2617,2.6648,0
0,2.2689,2.6602,0
0,2.2695,2.6597,0
0,2.2734,2.6571,0


==> SyntheticNN_Phi_150.tex <==
phi,x,y,z
0,1.9375,1.7496,0
0,1.9345,1.75,0
0,1.9414,1.7491,0
0,1.9453,1.7486,0
0,1.9492,1.7482,0
0,1.9531,1.7478,0
0,1.957,1.7475,0
0,1.9609,1.7471,0
0,1.9648,1.7468,0
0,1.9688,1.7466,0
0,1.9727,1.7463,0
0,1.9766,1.7461,0
0,1.9805,1.7459,0
0,1.9769,1.7461,0
0,1.9844,1.7458,0
0,1.9883,1.7457,0
0,1.9922,1.7456,0
0,1.9961,1.7455,0
0,2,1.7455,0
0,1.6875,1.8592,0
0,1.6873,1.8594,0
0,1.6719,1.8728,0
0,1.6694,1.875,0
0,1.6797,1.8658,0
0,1.6781,1.8672,0
0,1.6836,1.8625,0
0,1.6827,1.8633,0
0,1.6758,1.8693,0
0,1.6737,1.8711,0
0,1.7188,1.8352,0
0,1.7178,1.8359,0
0,1.7109,1.8409,0
0,1.7071,1.8438,0
0,1.7148,1.838,0
0,1.7123,1.8398,0
0,1.7305,1.8272,0
0,1.7291,1.8281,0
0,1.7344,1.8247,0
0,1.7422,1.8197,0
0,1.7412,1.8203,0
0,1.75,1.8149,0
0,1.7475,1.8164,0
0,1.7461,1.8173,0
0,1.7383,1.8221,0
0,1.735,1.8242,0
0,1.7266,1.8298,0
0,1.7234,1.832,0
0,1.7227,1.8325,0
0,1.7031,1.8467,0
0,1.7019,1.8477,0
0,1.6992,1.8498,0
0,1.6969,1.8516,0
0,1.6953,1.8528,0
0,1.6921,1.8555,0
0,1.6914,1.856,0
0,1.707,1.8438,0
0,1.625,1.9214,0
0,1.6246,1.9219,0
0,1.6213,1.9258,0
0,1.6211,1.9261,0
0,1.6182,1.9297,0
0,1.6172,1.9309,0
0,1.615,1.9336,0
0,1.6133,1.9358,0
0,1.612,1.9375,0
0,1.5938,1.9627,0
0,1.5923,1.9648,0
0,1.5898,1.9686,0
0,1.5897,1.9688,0
0,1.6094,1.9409,0
0,1.609,1.9414,0
0,1.6061,1.9453,0
0,1.6016,1.9515,0
0,1.6004,1.9531,0
0,1.6055,1.9461,0
0,1.6032,1.9492,0
0,1.5977,1.957,0
0,1.5977,1.957,0
0,1.595,1.9609,0
0,1.5859,1.9746,0
0,1.5847,1.9766,0
0,1.5872,1.9727,0
0,1.5823,1.9805,0
0,1.582,1.9809,0
0,1.5799,1.9844,0
0,1.5781,1.9873,0
0,1.5775,1.9883,0
0,1.5753,1.9922,0
0,1.5742,1.994,0
0,1.573,1.9961,0
0,1.5708,2,0
0,1.6562,1.8875,0
0,1.6531,1.8906,0
0,1.6406,1.9037,0
0,1.6383,1.9062,0
0,1.6484,1.8954,0
0,1.6455,1.8984,0
0,1.6523,1.8914,0
0,1.6493,1.8945,0
0,1.6445,1.8995,0
0,1.6419,1.9023,0
0,1.6641,1.88,0
0,1.6611,1.8828,0
0,1.668,1.8763,0
0,1.6652,1.8789,0
0,1.6602,1.8837,0
0,1.6571,1.8867,0
0,1.6328,1.9123,0
0,1.6313,1.9141,0
0,1.6367,1.9079,0
0,1.6347,1.9102,0
0,1.6289,1.9168,0
0,1.6279,1.918,0
0,1.7578,1.8103,0
0,1.7541,1.8125,0
0,1.7617,1.8081,0
0,1.7609,1.8086,0
0,1.7656,1.8059,0
0,1.7695,1.8038,0
0,1.7679,1.8047,0
0,1.7734,1.8017,0
0,1.7773,1.7997,0
0,1.7753,1.8008,0
0,1.7812,1.7977,0
0,1.7852,1.7957,0
0,1.7829,1.7969,0
0,1.7891,1.7939,0
0,1.793,1.792,0
0,1.7909,1.793,0
0,1.7969,1.7902,0
0,1.8008,1.7884,0
0,1.7993,1.7891,0
0,1.8047,1.7867,0
0,1.8086,1.785,0
0,1.8081,1.7852,0
0,1.8125,1.7833,0
0,1.8203,1.7801,0
0,1.8175,1.7812,0
0,1.8281,1.7771,0
0,1.8274,1.7773,0
0,1.8242,1.7786,0
0,1.8398,1.7728,0
0,1.838,1.7734,0
0,1.8438,1.7714,0
0,1.832,1.7756,0
0,1.8359,1.7742,0
0,1.8633,1.7652,0
0,1.862,1.7656,0
0,1.8672,1.7641,0
0,1.8711,1.763,0
0,1.875,1.762,0
0,1.8516,1.7689,0
0,1.8495,1.7695,0
0,1.8477,1.7701,0
0,1.8555,1.7676,0
0,1.8594,1.7664,0
0,1.8164,1.7817,0
0,1.7539,1.8126,0
0,1.8789,1.7609,0
0,1.8759,1.7617,0
0,1.8828,1.7599,0
0,1.8867,1.759,0
0,1.8906,1.7581,0
0,1.8945,1.7572,0
0,1.8917,1.7578,0
0,1.8984,1.7563,0
0,1.9023,1.7555,0
0,1.9062,1.7547,0
0,1.9141,1.7532,0
0,1.9104,1.7539,0
0,1.9102,1.754,0
0,1.918,1.7525,0
0,1.9219,1.7519,0
0,1.9258,1.7513,0
0,1.9297,1.7507,0
0,1.9336,1.7501,0
0,2.0039,1.7455,0
0,2.0078,1.7456,0
0,2.0117,1.7457,0
0,2.0156,1.7458,0
0,2.0195,1.7459,0
0,2.0231,1.7461,0
0,2.0234,1.7461,0
0,2.0273,1.7463,0
0,2.0312,1.7466,0
0,2.0352,1.7468,0
0,2.0391,1.7471,0
0,2.043,1.7475,0
0,2.0469,1.7478,0
0,2.0508,1.7482,0
0,2.0547,1.7486,0
0,2.0586,1.7491,0
0,2.0625,1.7496,0
0,2.0655,1.75,0
0,2.0664,1.7501,0
0,2.0703,1.7507,0
0,2.0742,1.7513,0
0,2.0781,1.7519,0
0,2.082,1.7525,0
0,2.0859,1.7532,0
0,2.0895,1.7539,0
0,2.0898,1.754,0
0,2.0938,1.7547,0
0,2.0977,1.7555,0
0,2.1016,1.7563,0
0,2.1055,1.7572,0
0,2.1082,1.7578,0
0,2.1094,1.7581,0
0,2.1133,1.759,0
0,2.1172,1.76,0
0,2.1211,1.7609,0
0,2.124,1.7617,0
0,2.125,1.762,0
0,2.1289,1.763,0
0,2.1328,1.7641,0
0,2.1367,1.7653,0
0,2.1379,1.7656,0
0,2.1406,1.7664,0
0,2.1445,1.7676,0
0,2.1484,1.7689,0
0,2.1504,1.7695,0
0,2.1523,1.7702,0
0,2.1562,1.7715,0
0,2.1602,1.7728,0
0,2.1619,1.7734,0
0,2.1641,1.7742,0
0,2.168,1.7756,0
0,2.1719,1.7771,0
0,2.1725,1.7773,0
0,2.1758,1.7786,0
0,2.1797,1.7801,0
0,2.1825,1.7812,0
0,2.1836,1.7817,0
0,2.1875,1.7833,0
0,2.1914,1.785,0
0,2.1918,1.7852,0
0,2.1953,1.7867,0
0,2.1992,1.7884,0
0,2.2007,1.7891,0
0,2.2031,1.7902,0
0,2.207,1.792,0
0,2.2091,1.793,0
0,2.2109,1.7939,0
0,2.2148,1.7958,0
0,2.2171,1.7969,0
0,2.2188,1.7977,0
0,2.2227,1.7997,0
0,2.2247,1.8008,0
0,2.2266,1.8017,0
0,2.2305,1.8038,0
0,2.2321,1.8047,0
0,2.2344,1.8059,0
0,2.2383,1.8081,0
0,2.2391,1.8086,0
0,2.2422,1.8103,0
0,2.2459,1.8125,0
0,2.2461,1.8126,0
0,2.25,1.8149,0
0,2.2525,1.8164,0
0,2.2539,1.8173,0
0,2.2578,1.8197,0
0,2.2588,1.8203,0
0,2.2617,1.8221,0
0,2.265,1.8242,0
0,2.2656,1.8247,0
0,2.2695,1.8272,0
0,2.2709,1.8281,0
0,2.2734,1.8298,0
0,2.2766,1.832,0
0,2.2773,1.8325,0
0,2.2812,1.8352,0
0,2.2822,1.8359,0
0,2.2852,1.838,0
0,2.2877,1.8398,0
0,2.2891,1.8409,0
0,2.2929,1.8438,0
0,2.293,1.8438,0
0,2.2969,1.8467,0
0,2.2981,1.8477,0
0,2.3008,1.8498,0
0,2.3031,1.8516,0
0,2.3047,1.8528,0
0,2.3079,1.8555,0
0,2.3086,1.856,0
0,2.3125,1.8592,0
0,2.3127,1.8594,0
0,2.3164,1.8625,0
0,2.3173,1.8633,0
0,2.3203,1.8658,0
0,2.3219,1.8672,0
0,2.3242,1.8693,0
0,2.3263,1.8711,0
0,2.3281,1.8728,0
0,2.3306,1.875,0
0,2.332,1.8763,0
0,2.3348,1.8789,0
0,2.3359,1.88,0
0,2.3389,1.8828,0
0,2.3398,1.8837,0
0,2.3429,1.8867,0
0,2.3438,1.8875,0
0,2.3468,1.8906,0
0,2.3477,1.8914,0
0,2.3507,1.8945,0
0,2.3516,1.8954,0
0,2.3545,1.8984,0
0,2.3555,1.8995,0
0,2.3581,1.9023,0
0,2.3594,1.9037,0
0,2.3618,1.9062,0
0,2.3633,1.9079,0
0,2.3653,1.9102,0
0,2.3672,1.9123,0
0,2.3687,1.9141,0
0,2.3711,1.9168,0
0,2.3721,1.918,0
0,2.375,1.9214,0
0,2.3754,1.9219,0
0,2.3787,1.9258,0
0,2.3789,1.9261,0
0,2.3818,1.9297,0
0,2.3828,1.9309,0
0,2.385,1.9336,0
0,2.3867,1.9358,0
0,2.388,1.9375,0
0,2.3906,1.9409,0
0,2.391,1.9414,0
0,2.3939,1.9453,0
0,2.3945,1.9461,0
0,2.3968,1.9492,0
0,2.3984,1.9515,0
0,2.3996,1.9531,0
0,2.4023,1.957,0
0,2.4024,1.957,0
0,2.4051,1.9609,0
0,2.4062,1.9627,0
0,2.4077,1.9648,0
0,2.4102,1.9685,0
0,2.4103,1.9688,0
0,2.4128,1.9727,0
0,2.4141,1.9746,0
0,2.4153,1.9766,0
0,2.4177,1.9805,0
0,2.418,1.9808,0
0,2.4201,1.9844,0
0,2.4219,1.9873,0
0,2.4225,1.9883,0
0,2.4247,1.9922,0
0,2.4258,1.994,0
0,2.427,1.9961,0
0,2.4292,2,0
0,1.5625,2.0156,0
0,1.5605,2.0195,0
0,1.5586,2.0234,0
0,1.5586,2.0235,0
0,1.5567,2.0273,0
0,1.5549,2.0312,0
0,1.5547,2.0316,0
0,1.5531,2.0352,0
0,1.5513,2.0391,0
0,1.5508,2.0402,0
0,1.5496,2.043,0
0,1.5479,2.0469,0
0,1.5469,2.0493,0
0,1.5462,2.0508,0
0,1.5446,2.0547,0
0,1.5431,2.0586,0
0,1.543,2.0588,0
0,1.5415,2.0625,0
0,1.5703,2.0009,0
0,1.5687,2.0039,0
0,1.5666,2.0078,0
0,1.5664,2.0081,0
0,1.5645,2.0117,0
0,1.5625,2.0156,0
0,1.5312,2.0916,0
0,1.5306,2.0938,0
0,1.5391,2.069,0
0,1.5386,2.0703,0
0,1.54,2.0664,0
0,1.5371,2.0742,0
0,1.5358,2.0781,0
0,1.5352,2.0799,0
0,1.5344,2.082,0
0,1.5331,2.0859,0
0,1.5318,2.0898,0
0,1.5294,2.0977,0
0,1.5282,2.1016,0
0,1.5273,2.1045,0
0,1.5271,2.1055,0
0,1.526,2.1094,0
0,1.5249,2.1133,0
0,1.5239,2.1172,0
0,1.5234,2.1188,0
0,1.5228,2.1211,0
0,1.5219,2.125,0
0,1.521,2.1289,0
0,1.5201,2.1328,0
0,1.5195,2.1351,0
0,1.5192,2.1367,0
0,1.5183,2.1406,0
0,1.5156,2.1545,0
0,1.5153,2.1562,0
0,1.5175,2.1445,0
0,1.5168,2.1484,0
0,1.516,2.1523,0
0,1.5146,2.1602,0
0,1.514,2.1641,0
0,1.5134,2.168,0
0,1.5128,2.1719,0
0,1.5123,2.1758,0
0,1.5117,2.1797,0
0,1.5117,2.1798,0
0,1.5112,2.1836,0
0,1.5108,2.1875,0
0,1.5104,2.1914,0
0,1.51,2.1953,0
0,1.5096,2.1992,0
0,1.5093,2.2031,0
0,1.509,2.207,0
0,1.5087,2.2109,0
0,1.5085,2.2148,0
0,1.5083,2.2188,0
0,1.5081,2.2227,0
0,1.508,2.2266,0
0,1.5078,2.2319,0
0,1.5078,2.2344,0
0,1.5078,2.2305,0
0,1.5077,2.2383,0
0,1.5077,2.2422,0
0,1.5077,2.2461,0
0,1.5077,2.25,0
0,1.5078,2.2539,0
0,1.5078,2.2545,0
0,1.5079,2.2578,0
0,1.508,2.2617,0
0,1.5082,2.2656,0
0,1.5084,2.2695,0
0,1.5086,2.2734,0
0,1.5089,2.2773,0
0,1.5091,2.2812,0
0,1.5094,2.2852,0
0,1.5098,2.2891,0
0,1.5102,2.293,0
0,1.5106,2.2969,0
0,1.511,2.3008,0
0,1.5115,2.3047,0
0,1.5117,2.3066,0
0,1.512,2.3086,0
0,1.5125,2.3125,0
0,1.5131,2.3164,0
0,1.5137,2.3203,0
0,1.5143,2.3242,0
0,1.5149,2.3281,0
0,1.5156,2.3319,0
0,1.5156,2.332,0
0,1.5164,2.3359,0
0,1.5171,2.3398,0
0,1.5179,2.3438,0
0,1.5187,2.3477,0
0,1.5195,2.3514,0
0,1.5196,2.3516,0
0,1.5205,2.3555,0
0,1.5214,2.3594,0
0,1.5223,2.3633,0
0,1.5233,2.3672,0
0,1.5234,2.3677,0
0,1.5243,2.3711,0
0,1.5254,2.375,0
0,1.5265,2.3789,0
0,1.5273,2.382,0
0,1.5276,2.3828,0
0,1.5287,2.3867,0
0,1.5299,2.3906,0
0,1.5311,2.3945,0
0,1.5312,2.3948,0
0,1.5324,2.3984,0
0,1.5337,2.4023,0
0,1.535,2.4062,0
0,1.5352,2.4066,0
0,1.5364,2.4102,0
0,1.5378,2.4141,0
0,1.5391,2.4175,0
0,1.5392,2.418,0
0,1.5407,2.4219,0
0,1.5422,2.4258,0
0,1.543,2.4276,0
0,1.5438,2.4297,0
0,1.5454,2.4336,0
0,1.5469,2.4372,0
0,1.547,2.4375,0
0,1.5487,2.4414,0
0,1.5504,2.4453,0
0,1.5508,2.4462,0
0,1.5521,2.4492,0
0,1.5539,2.4531,0
0,1.5547,2.4548,0
0,1.5557,2.457,0
0,1.5576,2.4609,0
0,1.5586,2.463,0
0,1.5595,2.4648,0
0,1.5615,2.4688,0
0,1.5625,2.4708,0
0,1.5635,2.4727,0
0,1.5655,2.4766,0
0,1.5664,2.4783,0
0,1.5676,2.4805,0
0,1.5697,2.4844,0
0,1.5703,2.4855,0
0,1.5719,2.4883,0
0,1.5741,2.4922,0
0,1.5742,2.4924,0
0,1.5763,2.4961,0
0,1.5781,2.4991,0
0,1.5787,2.5,0
0,1.581,2.5039,0
0,1.582,2.5056,0
0,1.5834,2.5078,0
0,1.5859,2.5117,0
0,1.5859,2.5118,0
0,1.5884,2.5156,0
0,1.5898,2.5178,0
0,1.591,2.5195,0
0,1.5936,2.5234,0
0,1.5938,2.5237,0
0,1.5962,2.5273,0
0,1.5977,2.5294,0
0,1.599,2.5312,0
0,1.6016,2.5349,0
0,1.6017,2.5352,0
0,1.6046,2.5391,0
0,1.6055,2.5403,0
0,1.6075,2.543,0
0,1.6094,2.5455,0
0,1.6104,2.5469,0
0,1.6133,2.5506,0
0,1.6134,2.5508,0
0,1.6165,2.5547,0
0,1.6172,2.5556,0
0,1.6196,2.5586,0
0,1.6211,2.5604,0
0,1.6228,2.5625,0
0,1.625,2.5651,0
0,1.6261,2.5664,0
0,1.6289,2.5697,0
0,1.6294,2.5703,0
0,1.6328,2.5742,0
0,1.6328,2.5742,0
0,1.6363,2.5781,0
0,1.6367,2.5786,0
0,1.6399,2.582,0
0,1.6406,2.5829,0
0,1.6435,2.5859,0
0,1.6445,2.587,0
0,1.6472,2.5898,0
0,1.6484,2.5911,0
0,1.651,2.5938,0
0,1.6523,2.5951,0
0,1.6549,2.5977,0
0,1.6562,2.599,0
0,1.6588,2.6016,0
0,1.6602,2.6029,0
0,1.6628,2.6055,0
0,1.6641,2.6066,0
0,1.667,2.6094,0
0,1.668,2.6103,0
0,1.6712,2.6133,0
0,1.6719,2.6139,0
0,1.6755,2.6172,0
0,1.6758,2.6174,0
0,1.6797,2.6208,0
0,1.68,2.6211,0
0,1.6836,2.6242,0
0,1.6845,2.625,0
0,1.6875,2.6275,0
0,1.6892,2.6289,0
0,1.6914,2.6308,0
0,1.6939,2.6328,0
0,1.6953,2.6339,0
0,1.6988,2.6367,0
0,1.6992,2.637,0
0,1.7031,2.6401,0
0,1.7038,2.6406,0
0,1.707,2.6431,0
0,1.709,2.6445,0
0,1.7109,2.646,0
0,1.7143,2.6484,0
0,1.7148,2.6488,0
0,1.7188,2.6516,0
0,1.7197,2.6523,0
0,1.7227,2.6544,0
0,1.7253,2.6562,0
0,1.7266,2.6571,0
0,1.7305,2.6597,0
0,1.7311,2.6602,0
0,1.7344,2.6623,0
0,1.7371,2.6641,0
0,1.7383,2.6648,0
0,1.7422,2.6673,0
0,1.7432,2.668,0
0,1.7461,2.6697,0
0,1.7496,2.6719,0
0,1.75,2.6721,0
0,1.7539,2.6744,0
0,1.7562,2.6758,0
0,1.7578,2.6767,0
0,1.7617,2.6789,0
0,1.763,2.6797,0
0,1.7656,2.6811,0
0,1.7695,2.6833,0
0,1.7701,2.6836,0
0,1.7734,2.6854,0
0,1.7773,2.6874,0
0,1.7775,2.6875,0
0,1.7812,2.6894,0
0,1.7852,2.6914,0
0,1.7852,2.6914,0
0,1.7891,2.6933,0
0,1.793,2.6951,0
0,1.7933,2.6953,0
0,1.7969,2.697,0
0,1.8008,2.6988,0
0,1.8018,2.6992,0
0,1.8047,2.7005,0
0,1.8086,2.7022,0
0,1.8107,2.7031,0
0,1.8125,2.7039,0
0,1.8164,2.7055,0
0,1.8202,2.707,0
0,1.8203,2.7071,0
0,1.8242,2.7086,0
0,1.8281,2.7101,0
0,1.8303,2.7109,0
0,1.832,2.7116,0
0,1.8359,2.713,0
0,1.8398,2.7144,0
0,1.8411,2.7148,0
0,1.8438,2.7158,0
0,1.8477,2.7171,0
0,1.8516,2.7184,0
0,1.8528,2.7188,0
0,1.8555,2.7196,0
0,1.8594,2.7208,0
0,1.8633,2.722,0
0,1.8656,2.7227,0
0,1.8672,2.7231,0
0,1.8711,2.7242,0
0,1.875,2.7253,0
0,1.8789,2.7263,0
0,1.8799,2.7266,0
0,1.8828,2.7273,0
0,1.8867,2.7283,0
0,1.8906,2.7292,0
0,1.8945,2.7301,0
0,1.8962,2.7305,0
0,1.8984,2.731,0
0,1.9023,2.7318,0
0,1.9062,2.7326,0
0,1.9102,2.7333,0
0,1.9141,2.734,0
0,1.9159,2.7344,0
0,1.918,2.7347,0
0,1.9219,2.7354,0
0,1.9258,2.736,0
0,1.9297,2.7366,0
0,1.9336,2.7372,0
0,1.9375,2.7377,0
0,1.9414,2.7382,0
0,1.9421,2.7383,0
0,1.9453,2.7387,0
0,1.9492,2.7391,0
0,1.9531,2.7395,0
0,1.957,2.7399,0
0,1.9609,2.7402,0
0,1.9648,2.7405,0
0,1.9688,2.7408,0
0,1.9727,2.741,0
0,1.9766,2.7412,0
0,1.9805,2.7414,0
0,1.9844,2.7415,0
0,1.9883,2.7416,0
0,1.9922,2.7417,0
0,1.9961,2.7418,0
0,2,2.7418,0
0,2.4297,2.0009,0
0,2.4313,2.0039,0
0,2.4334,2.0078,0
0,2.4336,2.0081,0
0,2.4355,2.0117,0
0,2.4375,2.0156,0
0,2.4375,2.0156,0
0,2.4395,2.0195,0
0,2.4414,2.0234,0
0,2.4414,2.0234,0
0,2.4433,2.0273,0
0,2.4452,2.0312,0
0,2.4453,2.0316,0
0,2.447,2.0352,0
0,2.4487,2.0391,0
0,2.4492,2.0402,0
0,2.4505,2.043,0
0,2.4521,2.0469,0
0,2.4531,2.0492,0
0,2.4538,2.0508,0
0,2.4554,2.0547,0
0,2.457,2.0586,0
0,2.457,2.0587,0
0,2.4585,2.0625,0
0,2.46,2.0664,0
0,2.4609,2.0689,0
0,2.4615,2.0703,0
0,2.4629,2.0742,0
0,2.4643,2.0781,0
0,2.4648,2.0798,0
0,2.4656,2.082,0
0,2.4669,2.0859,0
0,2.4682,2.0898,0
0,2.4688,2.0915,0
0,2.4695,2.0938,0
0,2.4707,2.0977,0
0,2.4718,2.1016,0
0,2.4727,2.1044,0
0,2.473,2.1055,0
0,2.4741,2.1094,0
0,2.4751,2.1133,0
0,2.4762,2.1172,0
0,2.4766,2.1187,0
0,2.4772,2.1211,0
0,2.4782,2.125,0
0,2.4791,2.1289,0
0,2.48,2.1328,0
0,2.4805,2.1349,0
0,2.4809,2.1367,0
0,2.4817,2.1406,0
0,2.4825,2.1445,0
0,2.4833,2.1484,0
0,2.484,2.1523,0
0,2.4844,2.1543,0
0,2.4847,2.1562,0
0,2.4854,2.1602,0
0,2.4861,2.1641,0
0,2.4867,2.168,0
0,2.4872,2.1719,0
0,2.4878,2.1758,0
0,2.4883,2.1795,0
0,2.4883,2.1797,0
0,2.4888,2.1836,0
0,2.4893,2.1875,0
0,2.4897,2.1914,0
0,2.4901,2.1953,0
0,2.4904,2.1992,0
0,2.4907,2.2031,0
0,2.491,2.207,0
0,2.4913,2.2109,0
0,2.4915,2.2148,0
0,2.4918,2.2188,0
0,2.4919,2.2227,0
0,2.4921,2.2266,0
0,2.4922,2.2304,0
0,2.4922,2.2305,0
0,2.4923,2.2344,0
0,2.4923,2.2383,0
0,2.4923,2.2422,0
0,2.4923,2.2461,0
0,2.4923,2.25,0
0,2.4921,2.2578,0
0,2.4922,2.2554,0
0,2.4922,2.2539,0
0,2.492,2.2617,0
0,2.4918,2.2656,0
0,2.4916,2.2695,0
0,2.4914,2.2734,0
0,2.4912,2.2773,0
0,2.4909,2.2812,0
0,2.4906,2.2852,0
0,2.4902,2.2891,0
0,2.4899,2.293,0
0,2.4894,2.2969,0
0,2.489,2.3008,0
0,2.4885,2.3047,0
0,2.488,2.3086,0
0,2.4883,2.3066,0
0,2.4875,2.3125,0
0,2.4869,2.3164,0
0,2.4863,2.3203,0
0,2.4857,2.3242,0
0,2.4851,2.3281,0
0,2.4844,2.332,0
0,2.4844,2.332,0
0,2.4836,2.3359,0
0,2.4829,2.3398,0
0,2.4821,2.3438,0
0,2.4813,2.3477,0
0,2.4804,2.3516,0
0,2.4805,2.3514,0
0,2.4795,2.3555,0
0,2.4786,2.3594,0
0,2.4777,2.3633,0
0,2.4767,2.3672,0
0,2.4757,2.3711,0
0,2.4766,2.3678,0
0,2.4746,2.375,0
0,2.4676,2.3984,0
0,2.4688,2.3949,0
0,2.4663,2.4023,0
0,2.465,2.4062,0
0,2.4736,2.3789,0
0,2.4724,2.3828,0
0,2.4727,2.3821,0
0,2.4713,2.3867,0
0,2.4701,2.3906,0
0,2.4689,2.3945,0
0,2.4636,2.4102,0
0,2.4648,2.4067,0
0,2.4622,2.4141,0
0,2.4608,2.418,0
0,2.4609,2.4176,0
0,2.4593,2.4219,0
0,2.4531,2.4375,0
0,2.4531,2.4373,0
0,2.4578,2.4258,0
0,2.4563,2.4297,0
0,2.457,2.4278,0
0,2.4547,2.4336,0
0,2.4366,2.4727,0
0,2.4375,2.4709,0
0,2.4346,2.4766,0
0,2.4325,2.4805,0
0,2.4336,2.4784,0
0,2.4304,2.4844,0
0,2.4214,2.5,0
0,2.4219,2.4992,0
0,2.4282,2.4883,0
0,2.4297,2.4856,0
0,2.426,2.4922,0
0,2.4237,2.4961,0
0,2.4258,2.4926,0
0,2.4514,2.4414,0
0,2.4497,2.4453,0
0,2.4479,2.4492,0
0,2.4492,2.4464,0
0,2.4462,2.4531,0
0,2.4443,2.457,0
0,2.4453,2.4549,0
0,2.4425,2.4609,0
0,2.4406,2.4648,0
0,2.4414,2.4631,0
0,2.4386,2.4688,0
0,2.0039,2.7418,0
0,2.0078,2.7417,0
0,2.0117,2.7416,0
0,2.0156,2.7415,0
0,2.0195,2.7414,0
0,2.0234,2.7412,0
0,2.0273,2.741,0
0,2.0312,2.7408,0
0,2.0352,2.7405,0
0,2.0391,2.7402,0
0,2.043,2.7399,0
0,2.0469,2.7395,0
0,2.0508,2.7391,0
0,2.0547,2.7387,0
0,2.058,2.7383,0
0,2.0586,2.7382,0
0,2.0625,2.7377,0
0,2.0842,2.7344,0
0,2.0859,2.7341,0
0,2.0898,2.7333,0
0,2.0938,2.7326,0
0,2.0664,2.7372,0
0,2.0703,2.7366,0
0,2.0742,2.736,0
0,2.0781,2.7354,0
0,2.082,2.7348,0
0,2.0977,2.7318,0
0,2.1016,2.731,0
0,2.1038,2.7305,0
0,2.1055,2.7301,0
0,2.1094,2.7292,0
0,2.1202,2.7266,0
0,2.1211,2.7263,0
0,2.125,2.7253,0
0,2.1133,2.7283,0
0,2.1172,2.7273,0
0,2.2226,2.6875,0
0,2.2227,2.6875,0
0,2.2266,2.6854,0
0,2.23,2.6836,0
0,2.2305,2.6833,0
0,2.2344,2.6812,0
0,2.2371,2.6797,0
0,2.2383,2.679,0
0,2.2422,2.6768,0
0,2.2439,2.6758,0
0,2.2461,2.6745,0
0,2.25,2.6722,0
0,2.1473,2.7188,0
0,2.1484,2.7184,0
0,2.1523,2.7171,0
0,2.1562,2.7158,0
0,2.1698,2.7109,0
0,2.1719,2.7102,0
0,2.159,2.7148,0
0,2.1602,2.7144,0
0,2.1641,2.7131,0
0,2.168,2.7116,0
0,2.1758,2.7087,0
0,2.1797,2.7071,0
0,2.1799,2.707,0
0,2.1836,2.7055,0
0,2.1875,2.7039,0
0,2.1289,2.7243,0
0,2.1328,2.7232,0
0,2.1345,2.7227,0
0,2.1367,2.722,0
0,2.1406,2.7208,0
0,2.1445,2.7196,0
0,2.1894,2.7031,0
0,2.1914,2.7022,0
0,2.1953,2.7006,0
0,2.1983,2.6992,0
0,2.1992,2.6988,0
0,2.2031,2.697,0
0,2.2068,2.6953,0
0,2.207,2.6952,0
0,2.2109,2.6933,0
0,2.2149,2.6914,0
0,2.2188,2.6895,0
0,2.2148,2.6914,0
0,2.374,2.5664,0
0,2.375,2.5652,0
0,2.3707,2.5703,0
0,2.3711,2.5698,0
0,2.3638,2.5781,0
0,2.3672,2.5743,0
0,2.3673,2.5742,0
0,2.3566,2.5859,0
0,2.3594,2.583,0
0,2.3492,2.5938,0
0,2.3516,2.5913,0
0,2.3529,2.5898,0
0,2.3555,2.5872,0
0,2.3603,2.582,0
0,2.3633,2.5787,0
0,2.3413,2.6016,0
0,2.3438,2.5992,0
0,2.3332,2.6094,0
0,2.3359,2.6068,0
0,2.3373,2.6055,0
0,2.3398,2.603,0
0,2.3246,2.6172,0
0,2.3281,2.614,0
0,2.3202,2.6211,0
0,2.3203,2.621,0
0,2.3156,2.625,0
0,2.3164,2.6243,0
0,2.3242,2.6175,0
0,2.3289,2.6133,0
0,2.332,2.6104,0
0,2.3453,2.5977,0
0,2.3477,2.5953,0
0,2.4039,2.5273,0
0,2.4062,2.5239,0
0,2.4011,2.5312,0
0,2.4023,2.5295,0
0,2.4191,2.5039,0
0,2.4167,2.5078,0
0,2.418,2.5057,0
0,2.4117,2.5156,0
0,2.4141,2.512,0
0,2.4142,2.5117,0
0,2.4091,2.5195,0
0,2.4102,2.518,0
0,2.4065,2.5234,0
0,2.3897,2.5469,0
0,2.3906,2.5457,0
0,2.3984,2.5352,0
0,2.3984,2.5351,0
0,2.3956,2.5391,0
0,2.3927,2.543,0
0,2.3945,2.5404,0
0,2.3867,2.5508,0
0,2.3867,2.5508,0
0,2.3836,2.5547,0
0,2.3805,2.5586,0
0,2.3828,2.5557,0
0,2.3773,2.5625,0
0,2.3789,2.5605,0
0,2.2804,2.6523,0
0,2.2812,2.6517,0
0,2.2748,2.6562,0
0,2.2773,2.6545,0
0,2.2963,2.6406,0
0,2.2969,2.6402,0
0,2.311,2.6289,0
0,2.3125,2.6276,0
0,2.3062,2.6328,0
0,2.3086,2.6309,0
0,2.3013,2.6367,0
0,2.3047,2.6341,0
0,2.3008,2.6372,0
0,2.2859,2.6484,0
0,2.2891,2.6461,0
0,2.2912,2.6445,0
0,2.293,2.6432,0
0,2.2852,2.649,0
0,2.2631,2.6641,0
0,2.2656,2.6624,0
0,2.2569,2.668,0
0,2.2578,2.6674,0
0,2.2505,2.6719,0
0,2.2539,2.6698,0
0,2.2617,2.6649,0
0,2.269,2.6602,0
0,2.2695,2.6598,0
0,2.2734,2.6572,0


==> syntheticAN.tex <==
time,velocity
0,0.0077
0.1000,0.0077
0.2000,0.0077
0.3000,0.0078
0.4000,0.0078
0.5000,0.0115
0.6000,0.0154
0.7000,0.0158
0.8000,0.0159
0.9000,0.0159
1.0000,0.0160
1.1000,0.0160
1.2000,0.0160
1.3000,0.0161
1.4000,0.0161
1.5000,0.0161
1.6000,0.0161
1.7000,0.0161
1.8000,0.0162
1.9000,0.0162
2.0000,0.0162
2.1000,0.0161
2.2000,0.0161
2.3000,0.0162
2.4000,0.0162
2.5000,0.0162
2.6000,0.0162
2.7000,0.0162
2.8000,0.0162
2.9000,0.0162
3.0000,0.0162
3.1000,0.0162
3.2000,0.0163
3.3000,0.0162
3.4000,0.0162
3.5000,0.0162
3.6000,0.0162
3.7000,0.0163
3.8000,0.0162
3.9000,0.0162
4.0000,0.0162
4.1000,0.0163
4.2000,0.0162
4.3000,0.0162
4.4000,0.0162
4.5000,0.0163
4.6000,0.0163
4.7000,0.0162
4.8000,0.0162
4.9000,0.0163
5.0000,0.0163
5.1000,0.0162
5.2000,0.0162
5.3000,0.0162
5.4000,0.0163
5.5000,0.0162
5.6000,0.0162
5.7000,0.0162
5.8000,0.0163
5.9000,0.0162
6.0000,0.0162
6.1000,0.0162
6.2000,0.0163
6.3000,0.0163
6.4000,0.0162
6.5000,0.0162
6.6000,0.0163
6.7000,0.0163
6.8000,0.0162
6.9000,0.0162
7.0000,0.0162
7.1000,0.0163
7.2000,0.0162
7.3000,0.0162
7.4000,0.0162
7.5000,0.0162
7.6000,0.0162
7.7000,0.0162
7.8000,0.0162
7.9000,0.0162
8.0000,0.0162
8.1000,0.0162
8.2000,0.0162
8.3000,0.0162
8.4000,0.0162
8.5000,0.0163
8.6000,0.0162
8.7000,0.0162
8.8000,0.0162
8.9000,0.0162
9.0000,0.0163
9.1000,0.0162
9.2000,0.0162
9.3000,0.0162
9.4000,0.0162
9.5000,0.0162
9.6000,0.0162
9.7000,0.0162
9.8000,0.0162
9.9000,0.0162
10.0000,0.0162
10.1000,0.0162
10.2000,0.0162
10.3000,0.0162
10.4000,0.0162
10.5000,0.0162
10.6000,0.0162
10.7000,0.0162
10.8000,0.0162
10.9000,0.0162
11.0000,0.0162
11.1000,0.0162
11.2000,0.0162
11.3000,0.0162
11.4000,0.0162
11.5000,0.0162
11.6000,0.0162
11.7000,0.0162
11.8000,0.0162
11.9000,0.0162
12.0000,0.0162
12.1000,0.0162
12.2000,0.0162
12.3000,0.0162
12.4000,0.0162
12.5000,0.0162
12.6000,0.0162
12.7000,0.0162
12.8000,0.0162
12.9000,0.0162
13.0000,0.0162
13.1000,0.0162
13.2000,0.0162
13.3000,0.0162
13.4000,0.0162
13.5000,0.0162
13.6000,0.0162
13.7000,0.0162
13.8000,0.0162
13.9000,0.0162
14.0000,0.0162
14.1000,0.0162
14.2000,0.0162
14.3000,0.0162
14.4000,0.0162
14.5000,0.0122
14.6000,0.0081
14.7000,0.0081
14.8000,0.0081
14.9000,0.0081
15.0000,0.0082


==> syntheticNN.tex <==
time,velocity
0,0.0076
0.1000,0.0077
0.2000,0.0078
0.3000,0.0078
0.4000,0.0078
0.5000,0.0115
0.6000,0.0155
0.7000,0.0159
0.8000,0.0159
0.9000,0.0159
1.0000,0.0160
1.1000,0.0160
1.2000,0.0160
1.3000,0.0161
1.4000,0.0161
1.5000,0.0161
1.6000,0.0161
1.7000,0.0161
1.8000,0.0162
1.9000,0.0162
2.0000,0.0162
2.1000,0.0161
2.2000,0.0162
2.3000,0.0162
2.4000,0.0162
2.5000,0.0162
2.6000,0.0162
2.7000,0.0162
2.8000,0.0162
2.9000,0.0162
3.0000,0.0162
3.1000,0.0162
3.2000,0.0162
3.3000,0.0162
3.4000,0.0162
3.5000,0.0162
3.6000,0.0162
3.7000,0.0163
3.8000,0.0162
3.9000,0.0162
4.0000,0.0162
4.1000,0.0162
4.2000,0.0163
4.3000,0.0162
4.4000,0.0162
4.5000,0.0163
4.6000,0.0163
4.7000,0.0162
4.8000,0.0162
4.9000,0.0162
5.0000,0.0163
5.1000,0.0163
5.2000,0.0162
5.3000,0.0162
5.4000,0.0163
5.5000,0.0162
5.6000,0.0162
5.7000,0.0162
5.8000,0.0162
5.9000,0.0163
6.0000,0.0162
6.1000,0.0162
6.2000,0.0163
6.3000,0.0163
6.4000,0.0162
6.5000,0.0162
6.6000,0.0163
6.7000,0.0163
6.8000,0.0163
6.9000,0.0162
7.0000,0.0162
7.1000,0.0163
7.2000,0.0162
7.3000,0.0162
7.4000,0.0162
7.5000,0.0162
7.6000,0.0162
7.7000,0.0162
7.8000,0.0162
7.9000,0.0162
8.0000,0.0162
8.1000,0.0162
8.2000,0.0162
8.3000,0.0162
8.4000,0.0162
8.5000,0.0163
8.6000,0.0162
8.7000,0.0162
8.8000,0.0162
8.9000,0.0162
9.0000,0.0163
9.1000,0.0162
9.2000,0.0162
9.3000,0.0162
9.4000,0.0162
9.5000,0.0162
9.6000,0.0162
9.7000,0.0162
9.8000,0.0162
9.9000,0.0162
10.0000,0.0162
10.1000,0.0162
10.2000,0.0162
10.3000,0.0162
10.4000,0.0162
10.5000,0.0162
10.6000,0.0162
10.7000,0.0162
10.8000,0.0162
10.9000,0.0162
11.0000,0.0162
11.1000,0.0162
11.2000,0.0162
11.3000,0.0162
11.4000,0.0162
11.5000,0.0162
11.6000,0.0162
11.7000,0.0162
11.8000,0.0162
11.9000,0.0163
12.0000,0.0162
12.1000,0.0162
12.2000,0.0162
12.3000,0.0162
12.4000,0.0163
12.5000,0.0162
12.6000,0.0162
12.7000,0.0162
12.8000,0.0162
12.9000,0.0162
13.0000,0.0162
13.1000,0.0162
13.2000,0.0162
13.3000,0.0162
13.4000,0.0162
13.5000,0.0162
13.6000,0.0162
13.7000,0.0162
13.8000,0.0162
13.9000,0.0162
14.0000,0.0162
14.1000,0.0162
14.2000,0.0162
14.3000,0.0162
14.4000,0.0162
14.5000,0.0121
14.6000,0.0081
14.7000,0.0081
14.8000,0.0081
14.9000,0.0081
15.0000,0.0080

